VirtSC: Combining Virtualization Obfuscation with Self-Checksumming

Self-checksumming (SC) is a tamper-proofing technique that ensures certain program segments (code) in memory hash to known values at runtime. SC has few restrictions on application and hence can protect a vast majority of programs. The code verification in SC requires computation of the expected hashes after compilation, as the machine-code is not known before. This means the expected hash values need to be adjusted in the binary executable, hence combining SC with other protections is limited due to this adjustment step. However, obfuscation protections are often necessary, as SC protections can be otherwise easily detected and disabled via pattern matching. In this paper, we present a layered protection using virtualization obfuscation, yielding an architecture-agnostic SC protection that requires no post-compilation adjustment. We evaluate the performance of our scheme using a dataset of 25 real-world programs (MiBench and 3 CLI games). Our results show that the SC scheme induces an average overhead of 43% for a complete protection (100% coverage). The overhead is tolerable for less CPU-intensive programs (e.g. games) and when only parts of programs (e.g. license checking) are protected. However, large overheads stemming from the virtualization obfuscation were encountered.

==> content/protection_coverage_table.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 2048            &         10 &             89   &               44.5 &         95.828  &           0.7 &             0   &     1.00499  &                   28.9 &                      0   &              49.2736  \\
 2048            &         25 &            214.7 &              216.5 &         97.6218 &           2.9 &             3   &     1.44568  &                   53.9 &                     44   &              41.2079  \\
 2048            &         50 &            338.1 &              325.5 &         68.2312 &           6.3 &             6.5 &     1.61555  &                   47.7 &                     46   &               7.78524 \\
 2048            &        100 &            781   &              781   &          0      &          16   &            16   &     0        &                   43.3 &                     46   &              19.0686  \\
 basicmath\_large &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_large &         10 &             36.6 &               30   &         37.7046 &           0.2 &             0   &     0.6      &                    0.6 &                      0   &               1.8     \\
 basicmath\_large &         25 &            205.4 &               33   &        239.135  &           0.4 &             0   &     0.489898 &                   25.2 &                      0   &              47.4569  \\
 basicmath\_large &         50 &            313.6 &              310   &        232.798  &           1.3 &             1   &     0.9      &                   55.2 &                     30   &              54.9123  \\
 basicmath\_large &        100 &            620   &              620   &          0      &           4   &             4   &     0        &                   15.6 &                      6   &              19.2     \\
 basicmath\_small &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_small &         10 &             96.3 &                0   &        136.237  &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_small &         25 &            124.2 &               60   &        156.95   &           0.6 &             0.5 &     0.663325 &                   46.8 &                     27   &              52.0861  \\
 basicmath\_small &         50 &            194.7 &              180   &         91.3445 &           1.2 &             1.5 &     0.87178  &                   54.6 &                     30   &              55.4765  \\
 basicmath\_small &        100 &            489   &              489   &          0      &           4   &             4   &     0        &                   45   &                      6   &              51.0705  \\
 bf              &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 bf              &         10 &            362.1 &              303.5 &        384.355  &           0.3 &             0   &     0.458258 &                  107.7 &                      0   &             164.514   \\
 bf              &         25 &           1226.2 &             1330   &        721.625  &           1.5 &             1   &     0.921954 &                  436.5 &                    359   &             382.705   \\
 bf              &         50 &           1408.5 &             1125.5 &        973.697  &           2.3 &             3   &     1.61555  &                  226.1 &                    161   &             287.42    \\
 bf              &        100 &           3629   &             3629   &          0      &           7   &             7   &     0        &                  685.4 &                    665   &             494.27    \\
 bitcnts         &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 bitcnts         &         10 &             90.3 &               70.5 &         76.5115 &           1.1 &             0.5 &     1.3      &                   37.4 &                     19.5 &              45.3436  \\
 bitcnts         &         25 &            165   &              156   &        101.784  &           2.7 &             3   &     1.61555  &                   32   &                     39   &              22.0363  \\
 bitcnts         &         50 &            329.8 &              347   &        126.509  &           6.4 &             6.5 &     1.95959  &                   62.2 &                     60   &              23.7815  \\
 bitcnts         &        100 &            692   &              692   &          0      &          14   &            14   &     0        &                   48.3 &                     40   &              27.4884  \\
 cjpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 cjpeg           &         10 &           5045.1 &             4596.5 &       1559.31   &          20   &            20   &     0        &                  188.3 &                    122.5 &             160.739   \\
 cjpeg           &         25 &          14255.9 &            14028.5 &       1542.25   &          50   &            40   &    27.2029   &                  366.7 &                    366.5 &             246.601   \\
 cjpeg           &         50 &          27621.5 &            28110.5 &       2447.67   &         118   &           130   &    55.4617   &                  818   &                    635.5 &             598.576   \\
 cjpeg           &        100 &          55565   &            55565   &          0      &         202   &           230   &    94        &                 1583.3 &                   1551   &             887.277   \\
 crc             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 crc             &         10 &             10.2 &                0   &         17.4402 &           0.1 &             0   &     0.3      &                    3.5 &                      0   &              10.5     \\
 crc             &         25 &             35.4 &               34   &         36.8489 &           0.3 &             0   &     0.640312 &                    6.9 &                      0   &              13.8018  \\
 crc             &         50 &             98.6 &              100.5 &         36.2414 &           1.5 &             1   &     0.921954 &                   37.4 &                     35   &              17.5852  \\
 crc             &        100 &            151   &              151   &          0      &           3   &             3   &     0        &                   47.1 &                     35   &              15.4366  \\
 dijkstra\_large  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 dijkstra\_large  &         10 &             58.5 &               40.5 &         66.1668 &           0.3 &             0   &     0.458258 &                   23.9 &                      0   &              40.9596  \\
 dijkstra\_large  &         25 &             74.9 &               70   &         65.3337 &           0.3 &             0   &     0.458258 &                   27.8 &                      0   &              43.9586  \\
 dijkstra\_large  &         50 &            209.9 &              203   &         60.2004 &           2.3 &             2   &     0.9      &                   80.5 &                     78   &              34.471   \\
 dijkstra\_large  &        100 &            331   &              331   &          0      &           5   &             5   &     0        &                   73.5 &                     70   &              45.6339  \\
 dijkstra\_small  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 dijkstra\_small  &         10 &             58.7 &               78   &         51.819  &           0.5 &             0   &     0.806226 &                   10.4 &                      0   &              20.7181  \\
 dijkstra\_small  &         25 &             78.7 &               62   &         69.0522 &           0.6 &             0   &     0.916515 &                   27.8 &                      0   &              40.3505  \\
 dijkstra\_small  &         50 &            191.3 &              170   &         82.4561 &           2   &             1.5 &     1.26491  &                   84.4 &                    100   &              39.1847  \\
 dijkstra\_small  &        100 &            331   &              331   &          0      &           5   &             5   &     0        &                   54.1 &                     50.5 &              49.6275  \\
 djpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 djpeg           &         10 &           4722.6 &             4561   &       1318.63   &          22   &            20   &     6        &                  103.9 &                     58.5 &             101.832   \\
 djpeg           &         25 &          13185.8 &            13354.5 &       2323.8    &          56   &            60   &    28        &                  463.5 &                    399.5 &             404.774   \\
 djpeg           &         50 &          26606.5 &            26530   &       1716.98   &          86   &            90   &    38        &                  615.8 &                    552.5 &             360.449   \\
 djpeg           &        100 &          53400   &            53400   &          0      &         190   &           130   &   110.363    &                 1229.5 &                    821.5 &             745.528   \\
 fft             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 fft             &         10 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 fft             &         25 &            217.5 &              287.5 &        149.342  &           1.1 &             0.5 &     1.3      &                   12.5 &                      7   &              13.1168  \\
 fft             &         50 &            377.5 &              374.5 &        256.072  &           2.2 &             2   &     1.77764  &                  115.7 &                     22   &             156.443   \\
 fft             &        100 &            757   &              757   &          0      &           6   &             6   &     0        &                   93.7 &                     33.5 &             130.397   \\
 patricia        &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 patricia        &         10 &             95.3 &                0   &        170.603  &           0.2 &             0   &     0.4      &                   31.9 &                      0   &              68.6214  \\
 patricia        &         25 &            247.2 &              168   &        263.121  &           0.5 &             0   &     0.806226 &                   34.3 &                      0   &              52.5777  \\
 patricia        &         50 &            660   &              663   &        227.553  &           2.3 &             2.5 &     0.9      &                  133.5 &                    120   &             119.265   \\
 patricia        &        100 &           1182   &             1182   &          0      &           5   &             5   &     0        &                  129.1 &                    103   &             109.899   \\
 qsort\_large     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_large     &         10 &             12.8 &                0   &         38.4    &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_large     &         25 &             38.4 &                0   &         58.657  &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_large     &         50 &            100.1 &              128   &         60.069  &           0.2 &             0   &     0.4      &                   25.6 &                      0   &              51.2     \\
 qsort\_large     &        100 &            163   &              163   &          0      &           1   &             1   &     0        &                  128   &                    128   &               0       \\
 qsort\_small     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_small     &         10 &              6.4 &                0   &         12.8    &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_small     &         25 &             22.2 &                0   &         33.9111 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_small     &         50 &             55   &               74   &         37.2048 &           0.1 &             0   &     0.3      &                    7.4 &                      0   &              22.2     \\
 qsort\_small     &        100 &            106   &              106   &          0      &           1   &             1   &     0        &                   74   &                     74   &               0       \\
 rawcaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawcaudio       &         10 &             60.6 &                0   &         93.2944 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawcaudio       &         25 &             86.9 &               34   &         93.9898 &           0.2 &             0   &     0.4      &                   34.4 &                      0   &              68.8     \\
 rawcaudio       &         50 &            229.8 &              234   &        140.926  &           0.7 &             1   &     0.640312 &                  116.7 &                    172   &              96.8659  \\
 rawcaudio       &        100 &            423   &              423   &          0      &           2   &             2   &     0        &                  190   &                    172   &              22.0454  \\
 rawdaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawdaudio       &         10 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawdaudio       &         25 &            108.6 &                0   &        168.378  &           0.5 &             0   &     0.806226 &                   51.6 &                      0   &              78.8203  \\
 rawdaudio       &         50 &            209.3 &              206   &         88.2961 &           0.7 &             1   &     0.640312 &                  107.7 &                    172   &              88.891   \\
 rawdaudio       &        100 &            423   &              423   &          0      &           2   &             2   &     0        &                  203.5 &                    217   &              20.6216  \\
 rijndael        &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rijndael        &         10 &            478.7 &                0   &        875.128  &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rijndael        &         25 &            830.1 &              341.5 &       1083.57   &           0.8 &             0   &     1.07703  &                   69.7 &                      0   &              96.3681  \\
 rijndael        &         50 &           3115.3 &             2598.5 &       1658.51   &           2   &             2   &     1.48324  &                  546.5 &                    169.5 &             841.354   \\
 rijndael        &        100 &           5891   &             5891   &          0      &           6   &             6   &     0        &                  772.3 &                    194.5 &             951.956   \\
 say             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 say             &         10 &            710.4 &              670.5 &        435.292  &           6.3 &             5.5 &     3.13209  &                   72.4 &                     46.5 &              81.4607  \\
 say             &         25 &           1829.9 &             1764.5 &        453.977  &          16.3 &            16.5 &     2.05183  &                   68.8 &                     48.5 &              51.2656  \\
 say             &         50 &           3787.3 &             3646.5 &        791.887  &          24   &            20   &     8        &                  183.2 &                     58   &             268.19    \\
 say             &        100 &           7171   &             7171   &          0      &          36   &            40   &    14.9666   &                  187.6 &                    123   &             175.971   \\
 search\_large    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 search\_large    &         10 &             28.7 &                0   &         44.5647 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 search\_large    &         25 &            171.4 &              120.5 &        136.688  &           1.1 &             1   &     1.13578  &                   46.4 &                     50.5 &              41.8884  \\
 search\_large    &         50 &            361   &              348.5 &        129.558  &           3.3 &             3.5 &     1.41774  &                   72.9 &                     98.5 &              41.6112  \\
 search\_large    &        100 &            861   &              861   &          0      &           9   &             9   &     0        &                   70.3 &                     73   &              60.2164  \\
 search\_small    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 search\_small    &         10 &            114.1 &              109   &         81.7208 &           0.6 &             0.5 &     0.663325 &                   38.3 &                     27.5 &              40.9098  \\
 search\_small    &         25 &            160.5 &              143   &        101.217  &           1.2 &             1   &     1.4      &                   43.7 &                     50.5 &              37.9264  \\
 search\_small    &         50 &            440.3 &              430   &        118.152  &           4.1 &             4.5 &     1.37477  &                   82.6 &                     91   &              37.4999  \\
 search\_small    &        100 &            861   &              861   &          0      &           9   &             9   &     0        &                  102.3 &                    106.5 &              27.7959  \\
 sha             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 sha             &         10 &            147.3 &               85.5 &        146.339  &           0.6 &             0   &     0.8      &                   20.4 &                      0   &              29.964   \\
 sha             &         25 &            149.3 &              113.5 &        137.89   &           1.3 &             1.5 &     0.781025 &                   83.4 &                     25   &             117.185   \\
 sha             &         50 &            327.3 &              360   &        179.539  &           2.9 &             3   &     1.37477  &                   98.8 &                     49   &             110.07    \\
 sha             &        100 &            665   &              665   &          0      &           7   &             7   &     0        &                   55.8 &                     71   &              25.4118  \\
 snake           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 snake           &         10 &             52   &               28   &         54.8361 &           0.3 &             0   &     0.458258 &                   23.3 &                      0   &              39.5728  \\
 snake           &         25 &            374.5 &              397.5 &        234.599  &           2.2 &             2   &     1.46969  &                   93.9 &                     43   &             118.531   \\
 snake           &         50 &            583.6 &              634   &        293.224  &           5.9 &             5.5 &     2.2561   &                  111.4 &                     34   &             129.397   \\
 snake           &        100 &           1101   &             1101   &          0      &          12   &            12   &     0        &                   82.2 &                     34   &              98.0416  \\
 susan           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 susan           &         10 &           1372.3 &              493.5 &       1488.49   &           0.9 &             1   &     0.7      &                 1081.9 &                    185.5 &            1247.04    \\
 susan           &         25 &           4078.8 &             4154.5 &       1987.87   &           4.4 &             4.5 &     1.35647  &                 1400.7 &                   1583   &            1146.64    \\
 susan           &         50 &           5679.5 &             6401.5 &       2476.68   &           7.4 &             7.5 &     2.37487  &                  264.2 &                    200   &             256.369   \\
 susan           &        100 &          12779   &            12779   &          0      &          18   &            18   &     0        &                  832.8 &                    272.5 &             986.79    \\
 tetris          &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 tetris          &         10 &             35.8 &               35.5 &         22.4268 &           0.3 &             0   &     0.458258 &                    2.1 &                      0   &               3.80657 \\
 tetris          &         25 &            194.9 &              171   &        140.598  &           2.1 &             2   &     1.81384  &                   44.6 &                     14   &              90.1423  \\
 tetris          &         50 &            342   &              410.5 &        150.877  &           5.1 &             5   &     0.830662 &                   23.8 &                     20.5 &              10.1074  \\
 tetris          &        100 &            649   &              649   &          0      &          12   &            12   &     0        &                   71.2 &                     13   &             120.055   \\
 toast           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 toast           &         10 &            996.1 &             1078   &        560.3    &           6   &             6   &     2.40832  &                  149.9 &                     49.5 &             271.044   \\
 toast           &         25 &           4127.5 &             4204.5 &        867.185  &          19   &            20   &     1.67332  &                   56.6 &                     37   &              43.5711  \\
 toast           &         50 &           7695.6 &             7706.5 &        926.582  &          32   &            40   &     9.79796  &                  431.6 &                     79   &             484.686   \\
 toast           &        100 &          15270   &            15270   &          0      &          54   &            60   &    22        &                  493.4 &                    318.5 &             434.351   \\
\hline
\end{tabular}
}
\end{table*}

==> content/protection_coverage_table_opt.tex <==
\begin{tabular}{|l|r|r|r|r|r|}
\hline
 program         &   virt\_inst\_mean &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean \\
\hline
 2048            &            781   &         128   &           127.5 &     2.82843  &                  699   \\\hline
 basicmath\_large &            620   &           9.8 &            10   &     0.4      &                  186   \\\hline
 basicmath\_small &            489   &           9.7 &            10   &     0.458258 &                  186   \\\hline
 bf              &           3629   &          27.3 &            27   &     0.640312 &                 3383   \\\hline
 bitcnts         &            692   &          99.1 &            99   &     1.97231  &                  669   \\\hline
 cjpeg           &          55565   &        7587.7 &          7587.5 &     2.83019  &                55396   \\\hline
 crc             &            151   &           6   &             6   &     0        &                  135   \\\hline
 dijkstra\_large  &            331   &          14.8 &            15   &     0.4      &                  304   \\\hline
 dijkstra\_small  &            331   &          15   &            15   &     0        &                  304   \\\hline
 djpeg           &          53400   &        7347.7 &          7348   &     2.83019  &                53204   \\\hline
 fft             &            757   &          20.8 &            21   &     0.4      &                  483   \\\hline
 patricia        &           1182   &          14.7 &            15   &     0.458258 &                  867   \\\hline
 qsort\_large     &            163   &           1   &             1   &     0        &                  128   \\\hline
 qsort\_small     &            106   &           1   &             1   &     0        &                   74   \\\hline
 rawcaudio       &            423   &           2.9 &             3   &     0.3      &                  389   \\\hline
 rawdaudio       &            423   &           3   &             3   &     0        &                  389   \\\hline
 rijndael        &           5891   &          20.6 &            21   &     0.663325 &                 5074   \\\hline
 say             &           7171   &        1267.8 &          1267   &     3.70945  &                 7135   \\\hline
 search\_large    &            861   &          43.4 &            43.5 &     1.11355  &                  741   \\\hline
 search\_small    &            861   &          42.7 &            42.5 &     0.781025 &                  741   \\\hline
 sha             &            665   &          26.9 &            27   &     0.7      &                  619   \\\hline
 snake           &           1101   &          74.5 &            74   &     0.921954 &                 1071   \\\hline
 susan           &          12779   &         160.3 &           160.5 &     1.48661  &                12760   \\\hline
 tetris          &            649   &          74.3 &            75   &     1.9      &                  564   \\\hline
 toast           &          15270   &        1645.3 &          1646   &     4.69148  &                15268   \\\hline
\hline
\end{tabular}

==> content/protection_coverage_table_secure.tex <==
\begin{tabular}{|l|r|r|r|r|r|}
\hline
 program         &   virt\_inst\_mean &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean \\
\hline
 2048            &            781   &         128.6 &           128.5 &     1.85472  &                  699   \\\hline
 basicmath\_large &            620   &           9.9 &            10   &     0.3      &                  186   \\\hline
 basicmath\_small &            489   &          10   &            10   &     0        &                  186   \\\hline
 bf              &           3629   &          27.1 &            27   &     0.830662 &                 3383   \\\hline
 bitcnts         &            692   &         100.2 &           101   &     2.44131  &                  669   \\\hline
 cjpeg           &          55565   &        7587.7 &          7587.5 &     1.95192  &                55396   \\\hline
 crc             &            151   &           5.9 &             6   &     0.3      &                  135   \\\hline
 dijkstra\_large  &            331   &          14.8 &            15   &     0.4      &                  304   \\\hline
 dijkstra\_small  &            331   &          14.5 &            14.5 &     0.5      &                  304   \\\hline
 djpeg           &          53400   &        7349.2 &          7347   &     3.6      &                53204   \\\hline
 fft             &            757   &          20.2 &            20   &     0.748331 &                  483   \\\hline
 patricia        &           1182   &          14.9 &            15   &     0.3      &                  867   \\\hline
 qsort\_large     &            163   &           1   &             1   &     0        &                  128   \\\hline
 qsort\_small     &            106   &           1   &             1   &     0        &                   74   \\\hline
 rawcaudio       &            423   &           3   &             3   &     0        &                  389   \\\hline
 rawdaudio       &            423   &           3   &             3   &     0        &                  389   \\\hline
 rijndael        &           5891   &          20.4 &            20   &     0.489898 &                 5074   \\\hline
 say             &           7171   &        1268.4 &          1268   &     3.13688  &                 7135   \\\hline
 search\_large    &            861   &          42.9 &            43   &     1.13578  &                  741   \\\hline
 search\_small    &            861   &          43.3 &            43   &     0.458258 &                  741   \\\hline
 sha             &            665   &          27.3 &            27.5 &     0.9      &                  619   \\\hline
 snake           &           1101   &          74.1 &            74   &     2.16564  &                 1071   \\\hline
 susan           &          12779   &         160.7 &           162   &     2.41039  &                12760   \\\hline
 tetris          &            649   &          74.4 &            74.5 &     1.8      &                  564   \\\hline
 toast           &          15270   &        1646.8 &          1647   &     2.44131  &                15268   \\
\hline
\end{tabular}

==> figures/eval/eval-conn0-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         10 &             83   &               50   &        104.101  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         25 &            144.7 &              150.5 &         75.6559 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         50 &            453.3 &              449   &         86.0198 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &        100 &            803   &              803   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         10 &            103.3 &                0   &        195.951  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         25 &            188.1 &              128   &        197.366  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         50 &            225.2 &              260.5 &        187.397  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &        100 &            649   &              649   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         10 &             50.8 &                0   &         97.6625 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         25 &            173.3 &              199   &        114.847  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         50 &            267.9 &              306   &        130.731  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &        100 &            538   &              538   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         10 &            181.8 &                0   &        383.621  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         25 &           1301.8 &             1364.5 &        893.715  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         50 &           2178.2 &             2226.5 &        721.246  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &        100 &           3667   &             3667   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         10 &             85.7 &               59.5 &         65.5836 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         25 &            126.6 &              108.5 &         61.0479 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         50 &            334.7 &              330   &         62.5748 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &        100 &            705   &              705   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         10 &           6072.7 &             6666.5 &       1334.48   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         25 &          14528.9 &            14222.5 &       1967.89   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         50 &          28937.5 &            29470.5 &       2783.75   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &        100 &          56735   &            56735   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         10 &             23.6 &               25   &         22.8307 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         25 &             16.8 &                0   &         23.8319 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         50 &             95.1 &              101.5 &         38.5083 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &        100 &            152   &              152   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         10 &             37.7 &                0   &         48.6622 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         25 &             75.1 &               73.5 &         41.9915 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         50 &            163.6 &              161.5 &         75.431  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &        100 &            338   &              338   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         10 &             28.8 &               14   &         32.2732 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         25 &             70.4 &               65   &         68.3904 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         50 &            188.9 &              222   &         69.7688 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &        100 &            338   &              338   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         10 &           5634.7 &             5285   &       1219.97   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         25 &          14125   &            14484   &       1839.49   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         50 &          28135.9 &            28175.5 &       1489.39   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &        100 &          54496   &            54496   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         10 &             43.4 &                0   &         92.7267 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         25 &            189.3 &               39   &        249.274  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         50 &            487.7 &              434.5 &        218.026  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &        100 &            760   &              760   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         10 &             33.8 &                0   &         70.7924 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         25 &            292.1 &              321   &        203.19   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         50 &            701.7 &              667.5 &        276.105  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &        100 &           1201   &             1201   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         10 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         25 &             56.8 &               35   &         58.75   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         50 &             79.5 &               83   &         52.4428 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &        100 &            166   &              166   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         10 &              7.5 &                0   &         22.5    &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         25 &             20.3 &                0   &         32.2492 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         50 &             61   &               75   &         33.5559 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &        100 &            107   &              107   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         10 &             74.3 &                0   &        106.903  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         25 &             98.4 &                0   &        134.006  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         50 &            244.4 &              242   &        144.777  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &        100 &            437   &              437   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         10 &              3.4 &                0   &         10.2    &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         25 &            108.6 &              106   &         98.5548 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         50 &            167.2 &              212   &        142.723  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &        100 &            437   &              437   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         10 &            605.3 &              443.5 &        352.169  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         25 &           1748.5 &             1701.5 &        334.06   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         50 &           3589.4 &             3709.5 &        820.058  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &        100 &           7447   &             7447   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         10 &            116.7 &               55.5 &        125.599  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         25 &            195.3 &              210.5 &        104.303  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         50 &            467.1 &              411   &         90.8267 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &        100 &            873   &              873   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         10 &             50.8 &               51   &         49.487  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         25 &            151.4 &              109   &        124.808  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         50 &            533.8 &              535   &        125.352  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &        100 &            873   &              873   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         10 &             74.8 &                0   &        121.997  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         25 &            206.5 &              158.5 &        131.804  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         50 &            273.2 &              229   &        157.039  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &        100 &            666   &              666   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         10 &             76.9 &               37   &         96.467  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         25 &            261.6 &              203   &        148.735  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         50 &            618.1 &              606.5 &        223.564  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &        100 &           1124   &             1124   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         10 &            525.6 &              183   &        882.862  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         25 &           3663.7 &             3175.5 &       2544.24   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         50 &           7510.7 &             7311   &       2035.66   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &        100 &          12996   &            12996   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         10 &             89   &               28   &        142.197  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         25 &            216.2 &              133   &        170.943  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         50 &            368.5 &              389   &        167.829  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &        100 &            669   &              669   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &          0 &              0   &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         10 &            949.5 &              712   &        746.399  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         25 &           3475.2 &             3093.5 &       1424.63   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         50 &           7871.4 &             8296   &       1783.31   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &        100 &          15374   &            15374   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
\hline
\end{tabular}

==> figures/eval/eval-conn10-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 2048            &         10 &             77.2 &               66   &         60.2757 &           0.8 &             0.5 &     0.979796 &                   13   &                      7   &               17.9889 \\
 2048            &         25 &            180.6 &              162   &        102.633  &           3.2 &             3.5 &     2.13542  &                   45.3 &                     37.5 &               47.5501 \\
 2048            &         50 &            370.1 &              376   &        124.767  &           6.8 &             7   &     1.53623  &                   32   &                     19   &               21.1424 \\
 2048            &        100 &            803   &              803   &          0      &          10   &            10   &     0        &                   54.4 &                     49   &               45.3921 \\
 basicmath\_large &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_large &         10 &             60.1 &                4.5 &        121.523  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_large &         25 &            166.9 &              190   &        148.894  &           0.4 &             0   &     0.663325 &                   43.7 &                      0   &               75.068  \\
 basicmath\_large &         50 &            395.6 &              426   &        151.007  &           1.6 &             2   &     1.0198   &                   44.5 &                     33   &               54.3475 \\
 basicmath\_large &        100 &            649   &              649   &          0      &           4   &             4   &     0        &                   41.5 &                      9   &               53.9541 \\
 basicmath\_small &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_small &         10 &             82   &                4.5 &        150.391  &           0.2 &             0   &     0.4      &                   24.7 &                      0   &               57.6612 \\
 basicmath\_small &         25 &            172   &              199   &        110.213  &           1.1 &             1   &     0.7      &                   80.7 &                     57   &               75.0014 \\
 basicmath\_small &         50 &            255.7 &              269   &        131.577  &           1.5 &             1   &     1.11803  &                   57.8 &                     33   &               69.8438 \\
 basicmath\_small &        100 &            538   &              538   &          0      &           4   &             4   &     0        &                   69.2 &                     57   &               63.8761 \\
 bf              &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bf              &         10 &            557.8 &               80.5 &        884.996  &           0.6 &             0   &     1.0198   &                  115.2 &                      0   &              295.184  \\
 bf              &         25 &           1122.7 &             1265   &        648.089  &           1.6 &             1.5 &     1.0198   &                  809.9 &                    989   &              427.978  \\
 bf              &         50 &           1431.8 &             1341.5 &        956.293  &           2.3 &             2.5 &     0.9      &                  426.4 &                    394   &              392.968  \\
 bf              &        100 &           3667   &             3667   &          0      &           7   &             7   &     0        &                  478.8 &                    361   &              426.937  \\
 bitcnts         &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bitcnts         &         10 &             87.3 &               73.5 &         67.7171 &           0.9 &             0.5 &     0.943398 &                   27.4 &                      5.5 &               37.3984 \\
 bitcnts         &         25 &            170.6 &              150.5 &         95.0434 &           2.6 &             2   &     1.95959  &                   44.7 &                     40   &               35.043  \\
 bitcnts         &         50 &            342.7 &              338.5 &         76.4605 &           5.8 &             5.5 &     1.6      &                   55.8 &                     41   &               25.4236 \\
 bitcnts         &        100 &            705   &              705   &          0      &          10   &            10   &     0        &                   35.8 &                     40.5 &               19.6204 \\
 cjpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 cjpeg           &         10 &           5698   &             5891.5 &       1061.63   &          21   &            20   &    10.4403   &                  177.7 &                    148   &              122.727  \\
 cjpeg           &         25 &          13715.2 &            13711   &       2110.98   &          46   &            50   &    20.5913   &                  513.8 &                    467.5 &              259.745  \\
 cjpeg           &         50 &          28337.9 &            28421   &       1442.94   &         103   &           120   &    53.1131   &                 1405.4 &                   1558.5 &             1037.64   \\
 cjpeg           &        100 &          56735   &            56735   &          0      &         208   &           155   &   125.044    &                 3191.9 &                   2734.5 &             2181.22   \\
 crc             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 crc             &         10 &              5.1 &                0   &         11.0494 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 crc             &         25 &             52.2 &               67   &         40.032  &           0.4 &             0   &     0.663325 &                   13.6 &                      0   &               22.4062 \\
 crc             &         50 &             82.7 &               93.5 &         45.2903 &           1.2 &             1.5 &     1.07703  &                   23.9 &                     34   &               21.6677 \\
 crc             &        100 &            152   &              152   &          0      &           3   &             3   &     0        &                   44.2 &                     35   &               14.9318 \\
 dijkstra\_large  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_large  &         10 &             48.5 &               14   &         55.7947 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_large  &         25 &             65.1 &               32.5 &         76.393  &           0.5 &             0   &     0.67082  &                   24.8 &                      0   &               41.9233 \\
 dijkstra\_large  &         50 &            169.3 &              125   &         99.7016 &           2.3 &             2   &     1.26886  &                   67.9 &                     62   &               35.876  \\
 dijkstra\_large  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   68.9 &                     62   &               44.2119 \\
 dijkstra\_small  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_small  &         10 &             57.3 &               39.5 &         63.8969 &           0.3 &             0   &     0.458258 &                   25   &                      0   &               41.6101 \\
 dijkstra\_small  &         25 &             69.7 &               62   &         39.7418 &           0.5 &             0   &     0.67082  &                   10.8 &                      0   &               20.7258 \\
 dijkstra\_small  &         50 &            165.9 &              159.5 &        101.856  &           2.1 &             2   &     1.57797  &                   61.1 &                     79   &               45.818  \\
 dijkstra\_small  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   64.5 &                     51   &               45.7477 \\
 djpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 djpeg           &         10 &           5256.4 &             4963.5 &       1751.2    &          20   &            20   &     8.94427  &                  263.5 &                    246   &              208.585  \\
 djpeg           &         25 &          13708.8 &            13482.5 &       1485.92   &          54   &            55   &    24.98     &                  694.6 &                    619.5 &              307.329  \\
 djpeg           &         50 &          27993.2 &            28535.5 &       1776.84   &          94   &           100   &    22.891    &                 1475.9 &                   1419   &              589.454  \\
 djpeg           &        100 &          54496   &            54496   &          0      &         235   &           250   &    58.0086   &                 3332.6 &                   3339.5 &             1342.3    \\
 fft             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 fft             &         10 &             43.7 &                0   &        104.931  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 fft             &         25 &            230.6 &              197.5 &        214.135  &           1.4 &             1   &     1.28062  &                   17.4 &                     17.5 &               13.7273 \\
 fft             &         50 &            350.1 &              375.5 &        225.857  &           2.4 &             2   &     1.28062  &                   55.9 &                     28.5 &              100.669  \\
 fft             &        100 &            760   &              760   &          0      &           6   &             6   &     0        &                   57.4 &                     27   &               99.7589 \\
 patricia        &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 patricia        &         10 &            204.1 &              166.5 &        209.589  &           0.1 &             0   &     0.3      &                   21.6 &                      0   &               64.8    \\
 patricia        &         25 &            285.6 &              174.5 &        303.353  &           0.8 &             0.5 &     0.979796 &                   88   &                      6   &              132.625  \\
 patricia        &         50 &            705.9 &              874   &        371.439  &           2   &             2   &     1.26491  &                  172.5 &                    105   &              177.005  \\
 patricia        &        100 &           1201   &             1201   &          0      &           5   &             5   &     0        &                  174.3 &                    113.5 &              141.069  \\
 qsort\_large     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         10 &              3.5 &                0   &         10.5    &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         25 &              3.5 &                0   &         10.5    &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         50 &             96.1 &              131   &         66.5198 &           0.3 &             0   &     0.458258 &                   39.3 &                      0   &               60.0317 \\
 qsort\_large     &        100 &            166   &              166   &          0      &           1   &             1   &     0        &                  131   &                    131   &                0      \\
 qsort\_small     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         10 &              7.5 &                0   &         22.5    &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         25 &             38.5 &               32   &         40.9542 &           0.2 &             0   &     0.4      &                   15   &                      0   &               30      \\
 qsort\_small     &         50 &             52.4 &               32   &         40.7559 &           0.3 &             0   &     0.458258 &                   22.5 &                      0   &               34.3693 \\
 qsort\_small     &        100 &            107   &              107   &          0      &           1   &             1   &     0        &                   75   &                     75   &                0      \\
 rawcaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawcaudio       &         10 &             22.5 &                0   &         67.5    &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawcaudio       &         25 &            152.3 &              178   &         96.9464 &           0.3 &             0   &     0.458258 &                   62.8 &                      0   &               96.6931 \\
 rawcaudio       &         50 &            215.9 &              212   &        133.81   &           0.8 &             1   &     0.748331 &                  106.8 &                    178   &               87.2018 \\
 rawcaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  206.2 &                    225   &               23.0252 \\
 rawdaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         10 &             84   &               17   &         97.5777 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         25 &            177.4 &              225   &        151.731  &           0.3 &             0   &     0.458258 &                   58.1 &                      0   &               89.5751 \\
 rawdaudio       &         50 &            149.7 &              178   &         77.3796 &           0.3 &             0   &     0.458258 &                   53.4 &                      0   &               81.5698 \\
 rawdaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  192.1 &                    178   &               21.5381 \\
 say             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 say             &         10 &            835.5 &              723   &        438.517  &           6.4 &             7   &     1.8      &                   70.8 &                     49.5 &               74.0241 \\
 say             &         25 &           1996.5 &             2144   &        702.373  &          13   &            10   &     4.58258  &                   92.9 &                     53   &               86.2733 \\
 say             &         50 &           3526.1 &             3619.5 &        806.845  &          19   &            20   &     8.30662  &                  164.2 &                    166   &              116.145  \\
 say             &        100 &           7447   &             7447   &          0      &          35   &            30   &    16.8819   &                  236.2 &                    176   &              148.975  \\
 search\_large    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_large    &         10 &            121.7 &              110   &        113.043  &           0.5 &             0   &     0.67082  &                   30.6 &                      0   &               42.1502 \\
 search\_large    &         25 &            236.5 &              245   &         93.2483 &           2   &             2   &     0.894427 &                   64.9 &                     77   &               37.4525 \\
 search\_large    &         50 &            432.7 &              473   &        140.85   &           3.9 &             4.5 &     1.51327  &                   95.8 &                     99.5 &               39.4    \\
 search\_large    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   99.2 &                    107.5 &               23.6169 \\
 search\_small    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_small    &         10 &             91.7 &              108   &         54.3618 &           0.3 &             0   &     0.458258 &                   14.8 &                      0   &               22.7543 \\
 search\_small    &         25 &            157.8 &               99.5 &        143.571  &           0.9 &             0.5 &     1.22066  &                   35.8 &                     28   &               37.1182 \\
 search\_small    &         50 &            432   &              418.5 &        108.998  &           3.8 &             4   &     0.979796 &                   90.1 &                    107.5 &               43.7892 \\
 search\_small    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   85.1 &                     84.5 &               46.6572 \\
 sha             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 sha             &         10 &             61.7 &               12.5 &        109.046  &           0.3 &             0   &     0.458258 &                   42   &                      0   &               93.884  \\
 sha             &         25 &            148.1 &               97.5 &        147.428  &           1.2 &             1   &     1.249    &                   78.2 &                     25   &              119.861  \\
 sha             &         50 &            314.2 &              266   &        191.452  &           3.2 &             3   &     1.66132  &                   44.5 &                     27.5 &               22.9271 \\
 sha             &        100 &            666   &              666   &          0      &           7   &             7   &     0        &                   88.8 &                     74   &               77.3393 \\
 snake           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 snake           &         10 &            151.9 &               75   &        143.241  &           0.5 &             0.5 &     0.5      &                   23.7 &                     14   &               31.9939 \\
 snake           &         25 &            342.9 &              292   &        242.619  &           2.6 &             2   &     1.11355  &                  131.4 &                     72   &              119.756  \\
 snake           &         50 &            597.5 &              569   &        262.919  &           6.6 &             7.5 &     2.05913  &                  108.4 &                     52   &              112.247  \\
 snake           &        100 &           1124   &             1124   &          0      &          10   &            10   &     0        &                  108.7 &                     39.5 &              112.667  \\
 susan           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 susan           &         10 &           1228.6 &              170.5 &       1486.41   &           0.5 &             0.5 &     0.5      &                  402.9 &                     32   &              792.899  \\
 susan           &         25 &           3088.1 &             3243   &       1808.81   &           3.5 &             3   &     1.68819  &                 1138.6 &                    851   &             1090.94   \\
 susan           &         50 &           6837   &             7477.5 &       1918.42   &           7.7 &             8.5 &     2.41039  &                  474.6 &                    159.5 &              683.857  \\
 susan           &        100 &          12996   &            12996   &          0      &          10   &            10   &     0        &                  772.5 &                    115   &              969.627  \\
 tetris          &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 tetris          &         10 &            122.4 &               44.5 &        139.595  &           0.5 &             0   &     0.67082  &                   67.6 &                      0   &              128.802  \\
 tetris          &         25 &            173.2 &               94   &        153.466  &           2.1 &             2   &     1.22066  &                   81.4 &                     26.5 &              122.351  \\
 tetris          &         50 &            423.2 &              489   &        159.617  &           6.3 &             7   &     1.34536  &                   87.3 &                     36   &              119.526  \\
 tetris          &        100 &            669   &              669   &          0      &          10   &            10   &     0        &                   52.9 &                     20   &               92.0928 \\
 toast           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 toast           &         10 &           1850.6 &             1739   &        989.505  &           8.7 &            10   &     1.95192  &                   74.3 &                     60   &               38.5332 \\
 toast           &         25 &           3881.4 &             4639   &       1709.21   &          12   &            10   &     4        &                  318.7 &                    126   &              440.723  \\
 toast           &         50 &           7302.5 &             7421   &       1440.1    &          25   &            25   &    12.0416   &                  470.2 &                    131.5 &              470.329  \\
 toast           &        100 &          15374   &            15374   &          0      &          49   &            60   &    25.4755   &                  417.2 &                    360.5 &              329.168  \\
\hline
\end{tabular}

==> figures/eval/eval-conn20-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 2048            &         10 &             88.2 &               85   &         55.9085 &           1.3 &             1.5 &     1.18743  &                   11.5 &                     14   &               12.508  \\
 2048            &         25 &            168.4 &              183.5 &         83.2517 &           2.7 &             3   &     1.61555  &                   24.3 &                     18.5 &               17.7429 \\
 2048            &         50 &            380.9 &              361.5 &        155.627  &           7.6 &             7.5 &     2.45764  &                   50.6 &                     47   &               45.3788 \\
 2048            &        100 &            803   &              803   &          0      &          16   &            16   &     0        &                   59.9 &                     45   &               40.5745 \\
 basicmath\_large &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_large &         10 &             26.5 &                0   &         57.8917 &           0.1 &             0   &     0.3      &                    5.7 &                      0   &               17.1    \\
 basicmath\_large &         25 &            107.8 &                9   &        160.845  &           0.4 &             0   &     0.8      &                    6.6 &                      0   &               17.0129 \\
 basicmath\_large &         50 &            328.8 &              388.5 &        211.579  &           1.3 &             1   &     1.00499  &                   49.3 &                     57   &               53.1056 \\
 basicmath\_large &        100 &            649   &              649   &          0      &           4   &             4   &     0        &                   54.8 &                      9   &               70.1096 \\
 basicmath\_small &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_small &         10 &             33.9 &                0   &         84.428  &           0.1 &             0   &     0.3      &                    0.9 &                      0   &                2.7    \\
 basicmath\_small &         25 &            199.2 &              128   &        182.231  &           0.8 &             1   &     0.748331 &                   19.8 &                      9   &               24.6366 \\
 basicmath\_small &         50 &            270.9 &              260.5 &        183.18   &           2.1 &             2   &     1.22066  &                   62.4 &                      9   &               83.5754 \\
 basicmath\_small &        100 &            538   &              538   &          0      &           4   &             4   &     0        &                   77.7 &                     57   &               76.1565 \\
 bf              &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bf              &         10 &            331.7 &                1   &        475.909  &           0.1 &             0   &     0.3      &                   98.9 &                      0   &              296.7    \\
 bf              &         25 &            601.3 &              211   &        748.678  &           0.8 &             0.5 &     0.979796 &                  194   &                      1   &              306.649  \\
 bf              &         50 &           1864.9 &             2174   &       1073.73   &           2.6 &             3   &     1.8      &                  350.5 &                    174   &              417.512  \\
 bf              &        100 &           3667   &             3667   &          0      &           7   &             7   &     0        &                  501.2 &                    361   &              330.379  \\
 bitcnts         &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bitcnts         &         10 &             74.3 &               65.5 &         65.5806 &           0.9 &             0.5 &     1.04403  &                   37.8 &                     20   &               46.0539 \\
 bitcnts         &         25 &            176.1 &              123.5 &        115.154  &           3   &             3   &     1.73205  &                   33.3 &                     34   &               10.8632 \\
 bitcnts         &         50 &            337.6 &              314   &        110.523  &           6.6 &             7   &     2.2      &                   45.1 &                     42   &               16.0028 \\
 bitcnts         &        100 &            705   &              705   &          0      &          14   &            14   &     0        &                   35.4 &                     40   &               13.8072 \\
 cjpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 cjpeg           &         10 &           5338.1 &             4828.5 &       1067.67   &          20   &            20   &     0        &                  161.4 &                    113.5 &              144.794  \\
 cjpeg           &         25 &          14312.7 &            14154.5 &       1333.71   &          52   &            50   &    28.5657   &                  289.8 &                    170.5 &              294.647  \\
 cjpeg           &         50 &          28954   &            28693.5 &       1678.34   &          96   &            90   &    54.9909   &                  573.8 &                    619.5 &              344.513  \\
 cjpeg           &        100 &          56735   &            56735   &          0      &         186   &           200   &    93.4024   &                 1596.2 &                   1686.5 &              866.953  \\
 crc             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 crc             &         10 &             25.2 &                8   &         33.0267 &           0.1 &             0   &     0.3      &                    3.4 &                      0   &               10.2    \\
 crc             &         25 &             36   &               34.5 &         40.6251 &           0.4 &             0   &     0.663325 &                   10.4 &                      0   &               15.8884 \\
 crc             &         50 &             53.9 &               68   &         37.292  &           0.6 &             0.5 &     0.663325 &                   23.8 &                     17   &               26.3051 \\
 crc             &        100 &            152   &              152   &          0      &           3   &             3   &     0        &                   44.2 &                     35   &               14.9318 \\
 dijkstra\_large  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_large  &         10 &             40.6 &                0   &         68.532  &           0.4 &             0   &     0.663325 &                   20.8 &                      0   &               42.1896 \\
 dijkstra\_large  &         25 &            133.7 &              114   &         59.5736 &           0.8 &             1   &     0.87178  &                   36.7 &                     21.5 &               42.5419 \\
 dijkstra\_large  &         50 &            169.9 &              192.5 &         80.224  &           2.2 &             2   &     0.87178  &                   46   &                     51   &               40.6473 \\
 dijkstra\_large  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   67.2 &                     62   &               44.1176 \\
 dijkstra\_small  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_small  &         10 &             31.4 &               21.5 &         32.0974 &           0.1 &             0   &     0.3      &                    4   &                      0   &               12      \\
 dijkstra\_small  &         25 &             76.2 &               40   &         78.6928 &           0.4 &             0   &     0.663325 &                   28.4 &                      0   &               45.0471 \\
 dijkstra\_small  &         50 &            172.1 &              182.5 &        108.648  &           2.1 &             2   &     1.37477  &                   47.1 &                     51   &               42.2811 \\
 dijkstra\_small  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   68.4 &                     70.5 &               45.1513 \\
 djpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 djpeg           &         10 &           5571   &             5473   &        922.633  &          24   &            20   &     8        &                  147   &                    102   &              143.298  \\
 djpeg           &         25 &          13190.6 &            13262   &       2181.39   &          44   &            40   &    19.5959   &                  440.8 &                    365   &              296.799  \\
 djpeg           &         50 &          27966.6 &            27899.5 &       1286.83   &          98   &            90   &    54.7357   &                  618.6 &                    618   &              358.436  \\
 djpeg           &        100 &          54496   &            54496   &          0      &         212   &           240   &   113.208    &                 1480.8 &                   1634   &              894.78   \\
 fft             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 fft             &         10 &             95.6 &               37   &        136.426  &           0.3 &             0   &     0.458258 &                   40   &                      0   &              105.751  \\
 fft             &         25 &            189.7 &              173.5 &        153.952  &           0.9 &             1   &     0.7      &                   51.5 &                     20.5 &              102.456  \\
 fft             &         50 &            412.6 &              388   &        246.019  &           2.7 &             3   &     1.73494  &                  120.7 &                     30   &              154.363  \\
 fft             &        100 &            760   &              760   &          0      &           6   &             6   &     0        &                   61.6 &                     33.5 &               98.4969 \\
 patricia        &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 patricia        &         10 &             88.6 &               58.5 &        126.717  &           0.1 &             0   &     0.3      &                   42.5 &                      0   &              127.5    \\
 patricia        &         25 &            249.2 &              222   &        207.7    &           0.6 &             0.5 &     0.663325 &                   74.7 &                     52.5 &               84.0155 \\
 patricia        &         50 &            686.6 &              609   &        248.502  &           2.3 &             2   &     1.1      &                  227.7 &                    169   &              170.769  \\
 patricia        &        100 &           1201   &             1201   &          0      &           5   &             5   &     0        &                  270.3 &                    320.5 &              167.627  \\
 qsort\_large     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         10 &             16.6 &                0   &         49.8    &           0.1 &             0   &     0.3      &                   13.1 &                      0   &               39.3    \\
 qsort\_large     &         25 &             49.8 &               35   &         55.0977 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         50 &             63.8 &               35   &         53.4075 &           0.1 &             0   &     0.3      &                   13.1 &                      0   &               39.3    \\
 qsort\_large     &        100 &            166   &              166   &          0      &           1   &             1   &     0        &                  131   &                    131   &                0      \\
 qsort\_small     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         10 &              3.2 &                0   &          9.6    &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         25 &             21.4 &                0   &         29.5269 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         50 &             67.4 &               75   &         38.3281 &           0.4 &             0   &     0.489898 &                   30   &                      0   &               36.7423 \\
 qsort\_small     &        100 &            107   &              107   &          0      &           1   &             1   &     0        &                   75   &                     75   &                0      \\
 rawcaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawcaudio       &         10 &             25.9 &                0   &         67.1364 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawcaudio       &         25 &            139.5 &              178   &        130.078  &           0.3 &             0   &     0.640312 &                   40.3 &                      0   &               81.2823 \\
 rawcaudio       &         50 &            176.9 &              212   &        159.88   &           0.7 &             0.5 &     0.781025 &                   93.7 &                     89   &               94.6383 \\
 rawcaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  201.5 &                    201.5 &               23.5    \\
 rawdaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         10 &             43.7 &                0   &         80.2297 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         25 &            139.2 &              123   &        141.255  &           0.4 &             0   &     0.489898 &                   80.6 &                      0   &               99.8271 \\
 rawdaudio       &         50 &            190.5 &              201.5 &        173.86   &           0.5 &             0   &     0.67082  &                   75.9 &                      0   &               93.845  \\
 rawdaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  201.5 &                    201.5 &               23.5    \\
 say             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 say             &         10 &            735.4 &              641.5 &        418.689  &           5.5 &             6   &     2.37697  &                  142   &                     73.5 &              180.995  \\
 say             &         25 &           1906.5 &             1979   &        613.523  &          17.5 &            17   &     2.01246  &                   83.9 &                     68.5 &               66.5935 \\
 say             &         50 &           3673.7 &             3535   &        591.81   &          24   &            20   &     8        &                   63.7 &                     33.5 &               71.1281 \\
 say             &        100 &           7447   &             7447   &          0      &          40   &            40   &    15.4919   &                  125.7 &                     65.5 &              111.085  \\
 search\_large    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_large    &         10 &            102.6 &              113   &         63.2585 &           0.3 &             0   &     0.458258 &                   22.5 &                      0   &               35.3079 \\
 search\_large    &         25 &            199.8 &              109.5 &        152.502  &           1.7 &             1   &     1.48661  &                   63.3 &                     77   &               43.6716 \\
 search\_large    &         50 &            442.1 &              528   &        181.379  &           3.7 &             4   &     1.79165  &                   74.6 &                     92   &               37.2108 \\
 search\_large    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   87.2 &                     92   &               31.8584 \\
 search\_small    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_small    &         10 &            128.7 &              107   &         76.7959 &           0.4 &             0   &     0.489898 &                   37.7 &                      0   &               51.7804 \\
 search\_small    &         25 &            227   &              229   &        123.461  &           1.6 &             1   &     1.28062  &                   71.4 &                     77   &               50.1262 \\
 search\_small    &         50 &            403.9 &              416.5 &        137.709  &           3.8 &             3.5 &     1.32665  &                   77.5 &                     92   &               33.5865 \\
 search\_small    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   76.5 &                     77   &               37.2431 \\
 sha             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 sha             &         10 &             49.5 &               35.5 &         61.3046 &           0.2 &             0   &     0.6      &                    7.4 &                      0   &               22.2    \\
 sha             &         25 &            174.2 &              120   &        111.052  &           1.4 &             1   &     1.68523  &                   35.7 &                     25   &               34.8484 \\
 sha             &         50 &            355   &              353   &        202.855  &           3.5 &             3.5 &     1.5      &                   75.6 &                     50.5 &               82.9195 \\
 sha             &        100 &            666   &              666   &          0      &           7   &             7   &     0        &                   40.4 &                     27.5 &               21.4392 \\
 snake           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 snake           &         10 &            136.6 &               89.5 &        138.577  &           0.7 &             0.5 &     0.781025 &                   72.4 &                     22   &              106.545  \\
 snake           &         25 &            295   &              229.5 &        216.999  &           2.1 &             2   &     1.57797  &                   43.4 &                     37   &               35.2908 \\
 snake           &         50 &            643.5 &              653   &        218.217  &           6.1 &             6   &     2.21133  &                   80.1 &                     44   &               97.2188 \\
 snake           &        100 &           1124   &             1124   &          0      &          12   &            12   &     0        &                   42.2 &                     44   &               19.964  \\
 susan           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 susan           &         10 &            424   &              112.5 &        490.155  &           0.5 &             0   &     0.67082  &                  193.9 &                      0   &              296.094  \\
 susan           &         25 &           3463.6 &             2890.5 &       2614.49   &           4   &             4   &     1.84391  &                 1193.6 &                   1056.5 &             1049.15   \\
 susan           &         50 &           6530.2 &             7188   &       2158.64   &           7.9 &             7.5 &     1.57797  &                  667.4 &                    276   &              871.656  \\
 susan           &        100 &          12996   &            12996   &          0      &          18   &            18   &     0        &                  610.8 &                    135   &              834.79   \\
 tetris          &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 tetris          &         10 &             89   &               36   &        126.092  &           0.3 &             0   &     0.458258 &                   38.1 &                      0   &               96.3353 \\
 tetris          &         25 &             81.7 &               55.5 &        108.054  &           1.5 &             1.5 &     1.20416  &                   40   &                      8   &               95.3132 \\
 tetris          &         50 &            353.1 &              464   &        206.347  &           5.3 &             5.5 &     1.73494  &                   85.6 &                     35   &              120.05   \\
 tetris          &        100 &            669   &              669   &          0      &          12   &            12   &     0        &                   50.2 &                     18.5 &               92.3448 \\
 toast           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 toast           &         10 &           1434.2 &             1284.5 &        931.088  &           8.8 &             9   &     2.95973  &                  128.9 &                     37   &              252.323  \\
 toast           &         25 &           3382.5 &             3419   &       1208.78   &          18.6 &            19.5 &     1.85472  &                  194.2 &                     51.5 &              311.997  \\
 toast           &         50 &           7856.2 &             8451   &       1610.3    &          26   &            20   &     9.16515  &                  125.2 &                     84   &              107.406  \\
 toast           &        100 &          15374   &            15374   &          0      &          56   &            60   &    23.3238   &                  521.9 &                    328.5 &              439.764  \\
\hline
\end{tabular}

==> figures/eval/eval-unopt-conn0-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         10 &           106.6  &               66   &         95.3884 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         25 &           203.65 &              171.5 &        123.441  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &         50 &           370.5  &              365   &        128.902  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 2048            &        100 &           803    &              803   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         10 &            68    &                4.5 &        104.089  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         25 &           179.05 &               61.5 &        202.996  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &         50 &           327.75 &              265   &        199.432  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_large &        100 &           649    &              649   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         10 &            44.75 &                0   &         97.2296 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         25 &            99.05 &               37.5 &        132.504  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &         50 &           250.35 &              273   &        195.662  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 basicmath\_small &        100 &           538    &              538   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         10 &           447.7  &              222   &        537.72   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         25 &           905.45 &              568   &        697.486  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &         50 &          1893.75 &             1846.5 &        816.855  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bf              &        100 &          3667    &             3667   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         10 &            74.05 &               74   &         48.4154 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         25 &           154.3  &              138   &         81.2909 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &         50 &           392.3  &              402   &        104.325  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 bitcnts         &        100 &           705    &              705   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         10 &          5811.15 &             5809.5 &       1505.94   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         25 &         14225.5  &            14104   &       1129.94   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &         50 &         29090.3  &            28300.5 &       2085.03   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 cjpeg           &        100 &         56735    &            56735   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         10 &            30.4  &               25   &         33.6636 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         25 &            39.75 &               35   &         33.8347 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &         50 &            74.55 &               68   &         37.5226 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 crc             &        100 &           152    &              152   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         10 &            44.5  &               29.5 &         53.2856 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         25 &           110.8  &              122.5 &         67.1443 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &         50 &           160.35 &              147   &         49.0003 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_large  &        100 &           338    &              338   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         10 &            27.4  &                0   &         47.991  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         25 &            77.3  &               54   &         71.345  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &         50 &           133.35 &              133.5 &         81.894  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 dijkstra\_small  &        100 &           338    &              338   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         10 &          5577.45 &             5707.5 &       1107.77   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         25 &         14007.3  &            14501.5 &       1587.36   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &         50 &         27362    &            27527.5 &       1272.42   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 djpeg           &        100 &         54496    &            54496   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         10 &            62.2  &               22   &        114.109  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         25 &           219.65 &              275   &        184.674  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &         50 &           435.65 &              420   &        162.351  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 fft             &        100 &           760    &              760   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         10 &           139.6  &               58.5 &        179.245  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         25 &           264.4  &              227.5 &        209.197  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &         50 &           526.45 &              492.5 &        207.99   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 patricia        &        100 &          1201    &             1201   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         10 &            18.35 &                0   &         44.9625 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         25 &            34.95 &                0   &         50.1692 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &         50 &            61.6  &               35   &         67.8015 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_large     &        100 &           166    &              166   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         10 &             5.35 &                0   &         17.4306 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         25 &            26.75 &                0   &         37.7715 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &         50 &            43.35 &               32   &         34.6299 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 qsort\_small     &        100 &           107    &              107   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         10 &            44.35 &                0   &         85.2574 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         25 &            94.2  &               34   &        100.925  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &         50 &           252.65 &              225   &        137.605  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawcaudio       &        100 &           437    &              437   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         10 &            15.7  &                0   &         39.6095 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         25 &           139.6  &              106   &        146.548  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &         50 &           194.3  &              178   &        143.249  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 rawdaudio       &        100 &           437    &              437   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         10 &           828.8  &              724.5 &        327.292  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         25 &          1638.3  &             1451.5 &        543.059  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &         50 &          3746.9  &             3690.5 &        712.826  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 say             &        100 &          7447    &             7447   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         10 &            62.7  &               56   &         67.799  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         25 &           254.1  &              286.5 &        145.037  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &         50 &           464.85 &              463.5 &        139.984  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_large    &        100 &           873    &              873   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         10 &            95.1  &               99.5 &         75.7911 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         25 &           205    &              169.5 &        144.026  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &         50 &           414.55 &              442.5 &        142.509  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 search\_small    &        100 &           873    &              873   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         10 &            58.95 &               25   &         98.1934 &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         25 &           189.7  &               98.5 &        163.912  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &         50 &           416.65 &              434   &        123.731  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 sha             &        100 &           666    &              666   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         10 &           116.75 &               30   &        155.132  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         25 &           357.15 &              394   &        215.34   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &         50 &           643.35 &              652.5 &        263.928  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 snake           &        100 &          1124    &             1124   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         10 &           874.45 &              144.5 &       1271.14   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         25 &          2584.05 &             2178.5 &       2003.77   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &         50 &          6036.5  &             6919.5 &       2554.78   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 susan           &        100 &         12996    &            12996   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         10 &            85    &               40   &        115.55   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         25 &           214    &              140   &        156.666  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &         50 &           393.4  &              466   &        166.219  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 tetris          &        100 &           669    &              669   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &          0 &             0    &                0   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         10 &          1711.55 &             1702.5 &        923.379  &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         25 &          4158.55 &             4083   &       1593.6    &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &         50 &          7558.75 &             7300   &       1509.76   &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
 toast           &        100 &         15374    &            15374   &          0      &             0 &               0 &            0 &                      0 &                        0 &                     0 \\
\hline
\end{tabular}

==> figures/eval/eval-unopt-conn10-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 2048            &         10 &             80   &               56.5 &         61.7301 &           1   &             0.5 &     1.34164  &                   13.2 &                      7   &              16.345   \\
 2048            &         25 &            180.2 &              145   &        124.36   &           3.1 &             3.5 &     1.57797  &                   41.2 &                     28   &              48.4434  \\
 2048            &         50 &            346.7 &              338.5 &         63.6852 &           6.6 &             7   &     1.0198   &                   31.2 &                     28.5 &              16.9458  \\
 2048            &        100 &            803   &              803   &          0      &          10   &            10   &     0        &                   32.8 &                     30.5 &              18.4813  \\
 basicmath\_large &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_large &         10 &             19.9 &                0   &         56.7635 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_large &         25 &            218.6 &              194.5 &        213.094  &           0.5 &             0.5 &     0.5      &                   76.9 &                      4.5 &              92.3823  \\
 basicmath\_large &         50 &            320.1 &              393   &        211.564  &           1.4 &             1   &     1.11355  &                   57.8 &                     33   &              69.8438  \\
 basicmath\_large &        100 &            649   &              649   &          0      &           4   &             4   &     0        &                   91   &                     57   &              82.7115  \\
 basicmath\_small &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 basicmath\_small &         10 &            109.4 &               42   &        118.688  &           0.3 &             0   &     0.458258 &                   12.3 &                      0   &              22.508   \\
 basicmath\_small &         25 &             86   &               57   &         92.8763 &           0.1 &             0   &     0.3      &                   19   &                      0   &              57       \\
 basicmath\_small &         50 &            246.3 &              208   &        154.966  &           1.5 &             1.5 &     1.0247   &                   48.2 &                      9   &              72.5407  \\
 basicmath\_small &        100 &            538   &              538   &          0      &           4   &             4   &     0        &                   64.4 &                     57   &              66.3675  \\
 bf              &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 bf              &         10 &            331.6 &              187   &        483.034  &           0.1 &             0   &     0.3      &                    0.2 &                      0   &               0.6     \\
 bf              &         25 &            575.6 &              188   &        723.603  &           0.3 &             0   &     0.458258 &                  198   &                      0   &             395.5     \\
 bf              &         50 &           1758   &             1480.5 &       1012.15   &           3.3 &             3.5 &     1.9      &                  287.8 &                    187   &             371.851   \\
 bf              &        100 &           3667   &             3667   &          0      &           7   &             7   &     0        &                  384.1 &                    274   &             412.888   \\
 bitcnts         &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 bitcnts         &         10 &             66.3 &               44.5 &         59.5215 &           0.7 &             0   &     1.1      &                   16.2 &                      0   &              25.9338  \\
 bitcnts         &         25 &            222.8 &              186.5 &        124.271  &           3.4 &             3   &     2.15407  &                   39.3 &                     39.5 &              20.8569  \\
 bitcnts         &         50 &            376.5 &              362   &         82.5303 &           6.5 &             7   &     1.43178  &                   54.7 &                     49   &              27.7238  \\
 bitcnts         &        100 &            705   &              705   &          0      &          10   &            10   &     0        &                   39.5 &                     32.5 &              29.9107  \\
 cjpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 cjpeg           &         10 &           5466.3 &             5775   &       1180.74   &          25   &            20   &    11.1803   &                  308.2 &                    239   &             215.345   \\
 cjpeg           &         25 &          14125.2 &            13899.5 &       1565.35   &          76   &            85   &    24.5764   &                  999   &                    893   &             493.262   \\
 cjpeg           &         50 &          28871.4 &            28867   &       1260.86   &         114   &           115   &    60.8605   &                 1772.5 &                   1849.5 &             941.606   \\
 cjpeg           &        100 &          56735   &            56735   &          0      &         145   &           150   &    74.8665   &                 2198.9 &                   2113   &            1216.68    \\
 crc             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 crc             &         10 &             10.2 &                0   &         21.6185 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 crc             &         25 &             20.3 &                0   &         34.5371 &           0.1 &             0   &     0.3      &                    3.5 &                      0   &              10.5     \\
 crc             &         50 &             67.6 &               60   &         41.8144 &           1   &             1   &     0.774597 &                   30.8 &                     35   &              23.5533  \\
 crc             &        100 &            152   &              152   &          0      &           3   &             3   &     0        &                   37.8 &                     35   &               9.74474 \\
 dijkstra\_large  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 dijkstra\_large  &         10 &             13.3 &                0   &         21.5316 &           0.1 &             0   &     0.3      &                    0.3 &                      0   &               0.9     \\
 dijkstra\_large  &         25 &            107.9 &              106   &         53.7168 &           0.9 &             1   &     0.943398 &                   48.2 &                     59.5 &              43.8265  \\
 dijkstra\_large  &         50 &            181   &              184.5 &         90.9824 &           1.8 &             2   &     1.32665  &                   77.4 &                    102.5 &              54.375   \\
 dijkstra\_large  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   61.2 &                     62   &              20.8365  \\
 dijkstra\_small  &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 dijkstra\_small  &         10 &             33.2 &                0   &         53.4674 &           0.1 &             0   &     0.3      &                    7.9 &                      0   &              23.7     \\
 dijkstra\_small  &         25 &             70.1 &               41.5 &         67.8844 &           0.5 &             0.5 &     0.5      &                   46   &                      1.5 &              57.1997  \\
 dijkstra\_small  &         50 &            140.4 &              155   &         84.2107 &           1.7 &             2   &     1.18743  &                   62.9 &                     59.5 &              56.3905  \\
 dijkstra\_small  &        100 &            338   &              338   &          0      &           5   &             5   &     0        &                   46   &                     51   &              40.6473  \\
 djpeg           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 djpeg           &         10 &           5049.2 &             4882   &        792.37   &          18   &            15   &     8.7178   &                  207.5 &                    142.5 &             178.777   \\
 djpeg           &         25 &          13798   &            13830.5 &       1169.7    &          56   &            60   &    22.4499   &                  756.4 &                    621   &             539.238   \\
 djpeg           &         50 &          26731   &            26927.5 &       1024.57   &          73   &            60   &    48.1768   &                 1183.2 &                    821.5 &             852.579   \\
 djpeg           &        100 &          54496   &            54496   &          0      &         255   &           300   &   103.658    &                 3156.8 &                   3426   &            1563.32    \\
 fft             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 fft             &         10 &             42.9 &               21   &         85.3937 &           0.1 &             0   &     0.3      &                    2.1 &                      0   &               6.3     \\
 fft             &         25 &             87.8 &               27   &        141.635  &           0.3 &             0   &     0.640312 &                    7.4 &                      0   &              14.8     \\
 fft             &         50 &            417.4 &              427   &        263.128  &           2.7 &             3   &     1.1      &                   91.9 &                     32   &             132.462   \\
 fft             &        100 &            760   &              760   &          0      &           6   &             6   &     0        &                   25.6 &                     24   &               8.52291 \\
 patricia        &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 patricia        &         10 &             67.2 &                6   &         97.518  &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 patricia        &         25 &            261.7 &              169   &        269.758  &           0.5 &             0   &     0.806226 &                   76.3 &                      0   &             135.627   \\
 patricia        &         50 &            731   &              711   &        296.312  &           2.7 &             2.5 &     1.1      &                  230.1 &                    216   &             140.42    \\
 patricia        &        100 &           1201   &             1201   &          0      &           5   &             5   &     0        &                  216.8 &                    216   &             113.873   \\
 qsort\_large     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_large     &         10 &             23.6 &                0   &         49.4332 &           0.1 &             0   &     0.3      &                   13.1 &                      0   &              39.3     \\
 qsort\_large     &         25 &             62.9 &               17.5 &         71.4807 &           0.2 &             0   &     0.4      &                   26.2 &                      0   &              52.4     \\
 qsort\_large     &         50 &             83   &               83   &         64.3273 &           0.2 &             0   &     0.4      &                   26.2 &                      0   &              52.4     \\
 qsort\_large     &        100 &            166   &              166   &          0      &           1   &             1   &     0        &                  131   &                    131   &               0       \\
 qsort\_small     &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_small     &         10 &             10.7 &                0   &         23.4608 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 qsort\_small     &         25 &             40.7 &               37.5 &         41.6942 &           0.1 &             0   &     0.3      &                    7.5 &                      0   &              22.5     \\
 qsort\_small     &         50 &             57.8 &               75   &         43.4023 &           0.3 &             0   &     0.458258 &                   22.5 &                      0   &              34.3693  \\
 qsort\_small     &        100 &            107   &              107   &          0      &           1   &             1   &     0        &                   75   &                     75   &               0       \\
 rawcaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawcaudio       &         10 &             35.6 &                0   &         71.2    &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawcaudio       &         25 &             82.7 &                0   &        136.785  &           0.2 &             0   &     0.6      &                   17.8 &                      0   &              53.4     \\
 rawcaudio       &         50 &            200.7 &              235.5 &        141.789  &           0.6 &             1   &     0.489898 &                  120.9 &                    178   &             100.379   \\
 rawcaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  201.5 &                    201.5 &              23.5     \\
 rawdaudio       &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawdaudio       &         10 &             74.3 &               17   &         99.4897 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 rawdaudio       &         25 &            105.2 &               34   &        129.632  &           0.1 &             0   &     0.3      &                   17.8 &                      0   &              53.4     \\
 rawdaudio       &         50 &            223.2 &              225   &        129.766  &           0.6 &             0.5 &     0.663325 &                   98.4 &                     89   &              99.7379  \\
 rawdaudio       &        100 &            437   &              437   &          0      &           2   &             2   &     0        &                  182.7 &                    178   &              14.1     \\
 say             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 say             &         10 &            813.7 &              723.5 &        466.444  &           6.4 &             6   &     2.24499  &                  135.4 &                     67.5 &             181.973   \\
 say             &         25 &           1805.3 &             1681.5 &        642.782  &          12   &            10   &     4        &                  150   &                     77   &             173.504   \\
 say             &         50 &           3933.3 &             4007.5 &        581.615  &          18   &            20   &     8.7178   &                  155.8 &                     99   &             167.571   \\
 say             &        100 &           7447   &             7447   &          0      &          46   &            45   &    22.891    &                  432.2 &                    400.5 &             230.698   \\
 search\_large    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 search\_large    &         10 &             85.2 &               92   &         74.5933 &           0.3 &             0   &     0.458258 &                   17.9 &                      0   &              28.2434  \\
 search\_large    &         25 &            234.5 &              279   &         86.9359 &           1.7 &             2   &     0.9      &                   66.3 &                     84.5 &              44.531   \\
 search\_large    &         50 &            393.1 &              397   &        124.416  &           3.7 &             3.5 &     1.00499  &                   89.6 &                     99.5 &              36.1309  \\
 search\_large    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   69.5 &                     84.5 &              38.5104  \\
 search\_small    &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 search\_small    &         10 &             87.7 &               53.5 &         95.1536 &           0.4 &             0   &     0.663325 &                   20.4 &                      0   &              32.5183  \\
 search\_small    &         25 &            246.6 &              214   &        166.834  &           1.7 &             1   &     1.48661  &                   61.3 &                     77   &              41.802   \\
 search\_small    &         50 &            505.4 &              579.5 &        152.593  &           4.9 &             6   &     1.7      &                   73.7 &                     66.5 &              22.579   \\
 search\_small    &        100 &            873   &              873   &          0      &           9   &             9   &     0        &                   91.3 &                    107   &              36.598   \\
 sha             &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 sha             &         10 &             32.5 &               35.5 &         30.8747 &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 sha             &         25 &            145.6 &              108   &        143.478  &           0.9 &             1   &     0.943398 &                   34.3 &                     25   &              33.097   \\
 sha             &         50 &            243.8 &              173.5 &        158.699  &           2.5 &             2.5 &     1.36015  &                   70.6 &                     50.5 &              84.9273  \\
 sha             &        100 &            666   &              666   &          0      &           7   &             7   &     0        &                   35.8 &                     25   &              19.1979  \\
 snake           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 snake           &         10 &            121.5 &               54.5 &        136.568  &           0.3 &             0   &     0.458258 &                   59   &                      0   &             110.856   \\
 snake           &         25 &            256   &              179   &        210.826  &           2.2 &             2   &     1.07703  &                   84.4 &                     66   &              70.419   \\
 snake           &         50 &            542.9 &              514   &        225.19   &           4.5 &             4.5 &     1.5      &                   69.8 &                     39.5 &              73.4572  \\
 snake           &        100 &           1124   &             1124   &          0      &          10   &            10   &     0        &                   61.1 &                     31.5 &              77.3672  \\
 susan           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 susan           &         10 &           1131.8 &              562   &       1189.7    &           1.4 &             1   &     1.42829  &                  500.9 &                    276   &             787.243   \\
 susan           &         25 &           3552   &             3319   &       2051.24   &           3.8 &             3   &     2.4      &                  963.2 &                    627   &             894.542   \\
 susan           &         50 &           5995.8 &             5803.5 &       2209.53   &           8.4 &             9   &     1.28062  &                  137.1 &                    128.5 &              66.742   \\
 susan           &        100 &          12996   &            12996   &          0      &          10   &            10   &     0        &                 1268.9 &                    744.5 &            1099.96    \\
 tetris          &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 tetris          &         10 &             64.6 &               27.5 &         96.5818 &           0.5 &             0   &     0.806226 &                   36.5 &                      0   &              96.4896  \\
 tetris          &         25 &            167.8 &               88.5 &        168.147  &           2.1 &             2.5 &     1.3      &                   75.8 &                     13   &             125.22    \\
 tetris          &         50 &            309.9 &              239.5 &        154.565  &           5.6 &             6   &     1.68523  &                   54.3 &                     20   &              91.1965  \\
 tetris          &        100 &            669   &              669   &          0      &          10   &            10   &     0        &                   26   &                     21   &              11.5758  \\
 toast           &          0 &              0   &                0   &          0      &           0   &             0   &     0        &                    0   &                      0   &               0       \\
 toast           &         10 &           1002.9 &              943   &        671.363  &           6.4 &             6   &     2.00998  &                  151.7 &                     73   &             210.105   \\
 toast           &         25 &           3426.6 &             2869.5 &       1314.16   &          12   &            10   &     4        &                  139.2 &                     83.5 &             115.345   \\
 toast           &         50 &           7084.6 &             7669   &       1311.1    &          19   &            20   &     8.30662  &                  407.8 &                     98   &             485.549   \\
 toast           &        100 &          15374   &            15374   &          0      &          37   &            40   &    23.2594   &                  344.3 &                    196.5 &             478.604   \\
\hline
\end{tabular}

==> figures/eval/eval-unopt-conn20-tbl.tex <==
\begin{tabular}{lrrrrrrrrrr}
\hline
 program         &   coverage &   virt\_inst\_mean &   virt\_inst\_median &   virt\_inst\_std &   guards\_mean &   guards\_median &   guards\_std &   protected\_insts\_mean &   protected\_insts\_median &   protected\_insts\_std \\
\hline
 2048            &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 2048            &         10 &             48.7 &               41   &        47.9355  &           0.5 &             0   &     0.921954 &                   12.7 &                      0   &               19.5092 \\
 2048            &         25 &            163.6 &              151.5 &        72.3411  &           3.1 &             3   &     1.13578  &                   25.4 &                     18.5 &               12.1754 \\
 2048            &         50 &            438.5 &              466.5 &       101.749   &           7.9 &             8   &     1.37477  &                   36.4 &                     40.5 &               19.0116 \\
 2048            &        100 &            803   &              803   &         0       &          16   &            16   &     0        &                   55.7 &                     50   &               43.8567 \\
 basicmath\_large &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_large &         10 &            102.4 &                4.5 &       151.487   &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_large &         25 &            259.6 &              194.5 &       239.223   &           1.1 &             1   &     1.04403  &                   37.9 &                      9   &               56.2538 \\
 basicmath\_large &         50 &            385.8 &              393   &       140.201   &           1.6 &             1.5 &     0.916515 &                   81.6 &                     57   &               74.0759 \\
 basicmath\_large &        100 &            649   &              649   &         0       &           4   &             4   &     0        &                   68.1 &                      9   &               81.0302 \\
 basicmath\_small &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_small &         10 &              2.7 &                0   &         4.12432 &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 basicmath\_small &         25 &            140.6 &               37.5 &       164.105   &           0.5 &             0   &     0.67082  &                   31.3 &                      0   &               57.3429 \\
 basicmath\_small &         50 &            166.4 &              190   &       149.433   &           0.5 &             0   &     0.806226 &                   12.3 &                      0   &               22.508  \\
 basicmath\_small &        100 &            538   &              538   &         0       &           4   &             4   &     0        &                   72.9 &                     33   &               78.7775 \\
 bf              &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bf              &         10 &            159.5 &               93.5 &       170.475   &           0.1 &             0   &     0.3      &                    0.2 &                      0   &                0.6    \\
 bf              &         25 &           1293.8 &             1397   &       776.043   &           1.7 &             2   &     1.34536  &                  207.3 &                    181.5 &              207.343  \\
 bf              &         50 &           1748.7 &             1685.5 &       781.677   &           2.3 &             2   &     0.781025 &                  600   &                    427   &              396.395  \\
 bf              &        100 &           3667   &             3667   &         0       &           7   &             7   &     0        &                  425.4 &                    274   &              386.04   \\
 bitcnts         &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 bitcnts         &         10 &             88.3 &               63.5 &        61.7188  &           1   &             0.5 &     1.18322  &                   28.3 &                     14   &               36.6798 \\
 bitcnts         &         25 &            175   &              186.5 &        54.5326  &           3   &             3   &     1.18322  &                   40.3 &                     42   &               15.5952 \\
 bitcnts         &         50 &            366.8 &              379.5 &       105.2     &           6.9 &             7   &     1.7      &                   38.3 &                     41   &               11.841  \\
 bitcnts         &        100 &            705   &              705   &         0       &          14   &            14   &     0        &                   57.9 &                     48   &               24.1762 \\
 cjpeg           &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 cjpeg           &         10 &           5834.2 &             6028   &      1166.31    &          28   &            20   &     9.79796  &                  236.6 &                    129   &              319.959  \\
 cjpeg           &         25 &          13422.8 &            13296   &      1155.27    &          48   &            40   &    16        &                  252.6 &                    199.5 &              162.178  \\
 cjpeg           &         50 &          27766.8 &            27736.5 &      2042.27    &         106   &           110   &    47.3709   &                  731.5 &                    620   &              469.204  \\
 cjpeg           &        100 &          56735   &            56735   &         0       &         188   &           150   &   127.185    &                 1410.1 &                   1288.5 &              926.111  \\
 crc             &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 crc             &         10 &             22   &                0   &        28.2206  &           0.1 &             0   &     0.3      &                    3.5 &                      0   &               10.5    \\
 crc             &         25 &             35.6 &               34   &        37.2376  &           0.3 &             0   &     0.458258 &                   10.3 &                      0   &               15.7356 \\
 crc             &         50 &             69.4 &               68   &        34.0094  &           0.9 &             1   &     0.830662 &                   24.2 &                     35   &               21.8119 \\
 crc             &        100 &            152   &              152   &         0       &           3   &             3   &     0        &                   41   &                     35   &               13.0077 \\
 dijkstra\_large  &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_large  &         10 &             36.6 &               29.5 &        39.8878  &           0.1 &             0   &     0.3      &                    0.3 &                      0   &                0.9    \\
 dijkstra\_large  &         25 &             55.9 &               73.5 &        39.8809  &           0.6 &             0.5 &     0.663325 &                   18.7 &                      1.5 &               28.6463 \\
 dijkstra\_large  &         50 &            132.8 &              119.5 &       105.568   &           1.5 &             1.5 &     1.43178  &                   42.6 &                     40   &               41.5384 \\
 dijkstra\_large  &        100 &            338   &              338   &         0       &           5   &             5   &     0        &                   73.5 &                     79   &               34.6273 \\
 dijkstra\_small  &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 dijkstra\_small  &         10 &             32.4 &               14   &        41.788   &           0.1 &             0   &     0.3      &                    6.2 &                      0   &               18.6    \\
 dijkstra\_small  &         25 &             87   &               86   &        57.1822  &           0.8 &             0.5 &     0.87178  &                   25.1 &                      1.5 &               41.7551 \\
 dijkstra\_small  &         50 &            171.7 &              176.5 &        80.1337  &           2.3 &             2   &     1.18743  &                   56.6 &                     40   &               49.2488 \\
 dijkstra\_small  &        100 &            338   &              338   &         0       &           5   &             5   &     0        &                   46.5 &                     62   &               39.883  \\
 djpeg           &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 djpeg           &         10 &           4885.6 &             4797.5 &      1182.17    &          24   &            20   &     8        &                  254   &                    244   &              190.069  \\
 djpeg           &         25 &          13444.4 &            13451   &      1397.61    &          48   &            40   &    18.3303   &                  522.3 &                    555   &              306.383  \\
 djpeg           &         50 &          26599.9 &            26413   &      1840.41    &          76   &            70   &    40.7922   &                  680.8 &                    523   &              437.316  \\
 djpeg           &        100 &          54496   &            54496   &         0       &         208   &           220   &   109.982    &                 1155.7 &                    948.5 &              761.729  \\
 fft             &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 fft             &         10 &             39.1 &                0   &       106.147   &           0.1 &             0   &     0.3      &                    1.4 &                      0   &                4.2    \\
 fft             &         25 &            186.2 &               36   &       220.756   &           0.6 &             0   &     0.8      &                   75.3 &                      0   &              140.604  \\
 fft             &         50 &            447.8 &              414   &       201.081   &           2.4 &             2.5 &     1.11355  &                  126.2 &                     37   &              150.618  \\
 fft             &        100 &            760   &              760   &         0       &           6   &             6   &     0        &                  158.6 &                     33.5 &              161.263  \\
 patricia        &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 patricia        &         10 &            107.3 &                0   &       143.339   &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 patricia        &         25 &            324.8 &              335.5 &       212.069   &           0.6 &             1   &     0.489898 &                   87   &                     58.5 &               92.9903 \\
 patricia        &         50 &            539.8 &              492.5 &       295.913   &           2.1 &             2   &     1.04403  &                  120.7 &                    105   &              118.688  \\
 patricia        &        100 &           1201   &             1201   &         0       &           5   &             5   &     0        &                  168.3 &                    122   &              139.823  \\
 qsort\_large     &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         10 &             39.3 &                0   &        60.0317  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         25 &             40.2 &               35   &        48.0225  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_large     &         50 &            122.3 &              148.5 &        63.0001  &           0.5 &             0.5 &     0.5      &                   65.5 &                     65.5 &               65.5    \\
 qsort\_large     &        100 &            166   &              166   &         0       &           1   &             1   &     0        &                  131   &                    131   &                0      \\
 qsort\_small     &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         10 &             20.3 &               16   &        23.6645  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         25 &             28.9 &               16   &        32.5129  &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 qsort\_small     &         50 &             61   &               75   &        40.0749  &           0.3 &             0   &     0.458258 &                   22.5 &                      0   &               34.3693 \\
 qsort\_small     &        100 &            107   &              107   &         0       &           1   &             1   &     0        &                   75   &                     75   &                0      \\
 rawcaudio       &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawcaudio       &         10 &             43.7 &                0   &        89.257   &           0.1 &             0   &     0.3      &                   22.5 &                      0   &               67.5    \\
 rawcaudio       &         25 &            111.2 &               89   &       112.688   &           0.1 &             0   &     0.3      &                   22.5 &                      0   &               67.5    \\
 rawcaudio       &         50 &            163.8 &              195   &       130.802   &           0.4 &             0   &     0.663325 &                   62.8 &                      0   &               96.6931 \\
 rawcaudio       &        100 &            437   &              437   &         0       &           2   &             2   &     0        &                  206.2 &                    225   &               23.0252 \\
 rawdaudio       &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         10 &             17.8 &                0   &        53.4     &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 rawdaudio       &         25 &            103.9 &              106   &        92.1851  &           0.1 &             0   &     0.3      &                   17.8 &                      0   &               53.4    \\
 rawdaudio       &         50 &            282.6 &              331   &       145.815   &           0.7 &             1   &     0.640312 &                  111.5 &                    178   &               92.0448 \\
 rawdaudio       &        100 &            437   &              437   &         0       &           2   &             2   &     0        &                  196.8 &                    178   &               23.0252 \\
 say             &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 say             &         10 &            724.7 &              629   &       415.678   &           5.9 &             6   &     2.42693  &                   68.6 &                     64   &               42.779  \\
 say             &         25 &           1472.9 &             1338   &       583.149   &          16.6 &            16   &     2.41661  &                  100.4 &                     35.5 &              176.136  \\
 say             &         50 &           3709.6 &             3652   &       918.985   &          20   &            20   &     0        &                   43   &                     26.5 &               45.8607 \\
 say             &        100 &           7447   &             7447   &         0       &          44   &            50   &    17.4356   &                  317.6 &                    208   &              292.067  \\
 search\_large    &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_large    &         10 &            131.4 &              146   &        82.0502  &           0.4 &             0   &     0.663325 &                   27   &                      0   &               43.2943 \\
 search\_large    &         25 &            229.3 &              242   &       118.714   &           1.6 &             1.5 &     1.11355  &                   67.5 &                     56   &               49.496  \\
 search\_large    &         50 &            452.6 &              445   &       124.494   &           4.2 &             4.5 &     1.46969  &                   88   &                    107   &               52.3202 \\
 search\_large    &        100 &            873   &              873   &         0       &           9   &             9   &     0        &                   66   &                     56   &               42.8416 \\
 search\_small    &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 search\_small    &         10 &             88.7 &               86.5 &        99.7086  &           0.5 &             0   &     0.921954 &                   17.9 &                      0   &               28.2434 \\
 search\_small    &         25 &            235.2 &              221   &       137.624   &           1.7 &             1.5 &     1.18743  &                   62.8 &                     66.5 &               36.3175 \\
 search\_small    &         50 &            422.8 &              399   &       157.361   &           3.4 &             3.5 &     1.42829  &                   96.1 &                    108   &               36.8088 \\
 search\_small    &        100 &            873   &              873   &         0       &           9   &             9   &     0        &                   69.1 &                     66.5 &               19.5113 \\
 sha             &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 sha             &         10 &             28.1 &               12.5 &        34.795   &           0.1 &             0   &     0.3      &                    2.5 &                      0   &                7.5    \\
 sha             &         25 &            141   &              101   &       143.193   &           1.3 &             1.5 &     1.00499  &                   46.9 &                     25   &               89.7914 \\
 sha             &         50 &            259.9 &              330.5 &       134.688   &           1.8 &             2   &     1.249    &                   90.5 &                     25   &              114.025  \\
 sha             &        100 &            666   &              666   &         0       &           7   &             7   &     0        &                   68.5 &                     27.5 &               84.4136 \\
 snake           &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 snake           &         10 &            167.8 &               72.5 &       215.144   &           0.9 &             0.5 &     0.943398 &                  105.9 &                     14   &              137.616  \\
 snake           &         25 &            331.5 &              405   &       193.337   &           2   &             2   &     1.41421  &                  183.3 &                    193.5 &              152.507  \\
 snake           &         50 &            491.3 &              565   &       237.814   &           3.9 &             4   &     1.44568  &                   98.6 &                     39.5 &              115.481  \\
 snake           &        100 &           1124   &             1124   &         0       &          12   &            12   &     0        &                  182.2 &                    193.5 &              136.274  \\
 susan           &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 susan           &         10 &           1044.9 &              516   &      1007.47    &           0.6 &             0.5 &     0.663325 &                  693   &                     47.5 &             1011.25   \\
 susan           &         25 &           3050.1 &             3244.5 &      1416.47    &           3.2 &             3   &     1.8868   &                 1263.8 &                    851   &             1197.85   \\
 susan           &         50 &           6533   &             6641   &      1726.01    &           8.3 &             8   &     2.05183  &                  516.5 &                    276   &              666.184  \\
 susan           &        100 &          12996   &            12996   &         0       &          18   &            18   &     0        &                  590.6 &                    249.5 &              730.08   \\
 tetris          &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 tetris          &         10 &             38.9 &               21   &        42.1769  &           0.6 &             0   &     0.916515 &                    6.9 &                      0   &               11.9369 \\
 tetris          &         25 &            122.2 &              122   &        99.2651  &           1.8 &             2   &     1.4      &                   12.4 &                      9.5 &               13.2831 \\
 tetris          &         50 &            461.5 &              454.5 &        49.0698  &           5   &             4.5 &     1.09545  &                  108.7 &                     14   &              142.177  \\
 tetris          &        100 &            669   &              669   &         0       &          12   &            12   &     0        &                   51.6 &                     17.5 &               92.1078 \\
 toast           &          0 &              0   &                0   &         0       &           0   &             0   &     0        &                    0   &                      0   &                0      \\
 toast           &         10 &           1305.9 &             1267.5 &       866.749   &           8.3 &             8   &     2.72213  &                  250.9 &                     65   &              404.115  \\
 toast           &         25 &           4137.4 &             3828.5 &      1607.38    &          18.5 &            20   &     2.01246  &                  235.3 &                     98.5 &              289.103  \\
 toast           &         50 &           7161.1 &             7145   &      1820.32    &          32   &            40   &     9.79796  &                  435.9 &                    110.5 &              540.756  \\
 toast           &        100 &          15374   &            15374   &         0       &          52   &            50   &    18.3303   &                  498   &                    249   &              449.867  \\
\hline
\end{tabular}
